Markovian Decentralized Ensemble Control for Demand Response

With the advancement in smart grid and smart energy devices, demand response becomes one of the most economic and feasible solutions to ease the load stress of the power grids during peak hours. In this work, we propose a fully decentralized ensemble control framework with consensus for demand response (DR) events and compatible control methods based on random policies. We show that under the consensus that is tailored to DR, our proposed decentralized control method yields the same optimality as the centralized control method in both myopic and multistage settings.

==> CDC 2022/literature_safe.tex <==



@article{lee2013assessment,
  title={Assessment of demand response and advanced metering},
  author={Richard Glick and others},
  journal={Federal Energy Regulatory Commission, Tech. Rep},
  year={2021}
}

% \bibitem{c1}
% Federal Energy Regulatory Commission, ``Assessment of demand response and advanced metering,” 2021. [Online]. Available: https://www.ferc.gov/legal/staff-reports/2021/DR-AM-Report2021.pdf

@article{ciso2020,
  title={2020 annual report on market issues \& performance},
  author={Eooo Hildebrandt and others},
  journal={California Independent System Operator},
  year={2020}
}

% \bibitem{c2}
% California Independent System Operator, ``2020 annual report on market issues \& performance,” 2020. [Online]. Available: http://www.caiso.com/Documents/2016AnnualReportonMarketIssues\\
% -andPerformance.pdf

% \bibitem{c3}
%  Communication Protocol Mapping Guide 1.0, OpenADR 2.0 to ANSI/CTA-2045-A
 
@inproceedings{chen2014individual,
  title={Individual risk in mean field control with application to automated demand response},
  author={Chen, Yue and others},
  booktitle={53rd IEEE Conf. on Decision and Control},
  pages={6425--6432},
  year={2014},
  organization={IEEE}
}

% @misc{openadr,
%   title = {OpenADR 2.0 Demand Response Program Implementation Guide},
%   howpublished = {\url{https://www.openadr.org/assets/openadr-drprogramguide-v1.0.pdf}}
% }


% @misc{condison,
%   title = {2011--2021 Demand Response event history book},
%   howpublished = {\url{https://www.coned.com/-/media/files/coned/documents/save-energy-money/rebates-incentives-tax-credits/smart-usage-rewards/demand-response-events.pdf?la=en.}}
% }

@article{meyn2015ancillary,
  title={Ancillary service to the grid using intelligent deferrable loads},
  author={Meyn, Sean P and others},
  journal={IEEE Trans. on Automatic Control},
  volume={60},
  number={11},
  pages={2847--2862},
  year={2015},
  publisher={IEEE}
}


@inproceedings{hao2012demand,
  title={How demand response from commercial buildings will provide the regulation needs of the grid},
  author={Hao, He and others},
  booktitle={2012 50th annual Allerton Conf. on communication, control, and computing (Allerton)},
  pages={1908--1913},
  year={2012},
  organization={IEEE}
}



@inproceedings{koch2011modeling,
  title={Modeling and control of aggregated heterogeneous thermostatically controlled loads for ancillary services},
  author={Koch, Stephan and others},
  booktitle={Proc. PSCC},
  pages={1--7},
  year={2011},
  organization={Citeseer}
}



@article{todorov2006linearly,
  title={Linearly-solvable Markov decision problems},
  author={Todorov, Emanuel},
  journal={Advances in neural information processing systems},
  volume={19},
  year={2006}
}

@incollection{chertkov2018ensemble,
  title={Ensemble control of cycling energy loads: Markov decision approach},
  author={Chertkov, Michael and others},
  booktitle={Energy Markets and Responsive Grids},
  pages={363--382},
  year={2018},
  publisher={Springer}
}


@article{hassan2020stochastic,
  title={Stochastic and distributionally robust load ensemble control},
  author={Hassan, Ali and others},
  journal={IEEE Trans. on Power Systems},
  volume={35},
  number={6},
  year={2020},
  publisher={IEEE}
}


@inproceedings{pop2019markov,
  title={A Markov process approach to ensemble control of smart buildings},
  author={Pop, Roman and others},
  booktitle={IEEE Milan PowerTech},
  pages={1--6},
  year={2019},
  organization={IEEE}
}






@article{wan2021distributed,
  title={Distributed algorithms for linearly-solvable optimal control in networked multi-agent systems},
  author={Wan, Neng and others},
  journal={arXiv preprint arXiv:2102.09104},
  year={2021}
}




@article{lobel2010distributed,
  title={Distributed subgradient methods for convex optimization over random networks},
  author={Lobel, Ilan and Ozdaglar, Asuman},
  journal={IEEE Trans. on Automatic Control},
  volume={56},
  number={6},
  pages={1291--1306},
  year={2010},
  publisher={IEEE}
}


@article{jakovetic2014fast,
  title={Fast distributed gradient methods},
  author={Jakoveti{\'c}, Du{\v{s}}an and others},
  journal={IEEE Trans. on Automatic Control},
  volume={59},
  number={5},
  pages={1131--1146},
  year={2014},
  publisher={IEEE}
}


@article{zhang2014online,
  title={Online optimal generation control based on constrained distributed gradient algorithm},
  author={Zhang, Wei and others},
  journal={IEEE Trans. on Power Systems},
  volume={30},
  number={1},
  pages={35--45},
  year={2014},
  publisher={IEEE}
}



@article{kullback1951information,
  title={On information and sufficiency},
  author={Kullback, Solomon and Leibler, Richard A},
  journal={The annals of mathematical statistics},
  volume={22},
  number={1},
  pages={79--86},
  year={1951},
  publisher={JSTOR}
}  
  
% \bibitem{KLD}
% S. Kullback, R. Leibler, ``On Information and Sufficiency," in \textit{The Annals of Mathematical Statistics}, 1951, 22(1), pp.79–86.
 
%  \bibitem{convexopt}
% S. Boyd, and L. Vandenberghe, ``Convex optimization," \textit{Cambridge university press}, 2004.

@book{greenberg2012introduction,
  title={Introduction to Bayesian econometrics},
  author={Greenberg, Edward},
  year={2012},
  publisher={Cambridge University Press}
}


@book{prohorov1969probability,
  title={Probability theory: basic concepts, limit theorems, random processes},
  author={Prohorov, Yurii Vasil'evich and others},
  volume={18},
  year={1969},
  publisher={Springer}
}





@article{hassan2020hierarchical,
  title={A hierarchical approach to multienergy demand response: From electricity to multienergy applications},
  author={Hassan, Ali and others},
  journal={Proc. of the IEEE},
  volume={108},
  number={9},
  pages={1457--1474},
  year={2020},
  publisher={IEEE}
}






% \bibitem{data1}
% A. Hassan, S. Acharya, M. Chertkov, D. Deka, and Y. Dvorkin, ``A hierarchical approach to multienergy demand response: From electricity to multienergy applications,” in \textit{Proc. of the IEEE}, 2020, 108(9), pp.1457-1474.



% \bibitem{data2}
% Consolidated Edison. [Online]. Available: https://www.coned.com/-/media/files/coned/documents/save-energy-money/rebates-incentives-tax-credits/smart-usage-rewards/demand-response-events.pdf?la=en



==> CDC 2022/set_margins.tex <==
\usepackage{placeins}
\newcommand{\subparagraph}{}
\usepackage{titlesec}

\titlespacing*{\section}{0pt}{5pt}{3pt}
\titlespacing*{\subsection}{0pt}{3pt}{0pt}
\titlespacing*{\subsubsection}{0pt}{3pt}{0pt}
\setlength{\parskip}{0cm}

\setlength{\belowdisplayskip}{4pt}
\setlength{\belowdisplayshortskip}{4pt}
\setlength{\abovedisplayskip}{4pt}
\setlength{\abovedisplayshortskip}{4pt}
% \setlength{\belowcaptionskip}{6pt}
% \setlength{\abovecaptionskip}{2pt}
\setlength{\textfloatsep}{8pt}
\setlength{\floatsep}{8pt}
% \setlength{\itemsep}{3pt}

==> literature_safe.tex <==



@article{lee2013assessment,
  title={Assessment of demand response and advanced metering},
  author={Richard Glick and others},
  journal={Federal Energy Regulatory Commission, Tech. Rep},
  year={2021}
}

% \bibitem{c1}
% Federal Energy Regulatory Commission, ``Assessment of demand response and advanced metering,” 2021. [Online]. Available: https://www.ferc.gov/legal/staff-reports/2021/DR-AM-Report2021.pdf

@article{ciso2020,
  title={2020 annual report on market issues \& performance},
  author={Eooo Hildebrandt and others},
  journal={California Independent System Operator},
  year={2020}
}

% \bibitem{c2}
% California Independent System Operator, ``2020 annual report on market issues \& performance,” 2020. [Online]. Available: http://www.caiso.com/Documents/2016AnnualReportonMarketIssues\\
% -andPerformance.pdf

% \bibitem{c3}
%  Communication Protocol Mapping Guide 1.0, OpenADR 2.0 to ANSI/CTA-2045-A
 
@inproceedings{chen2014individual,
  title={Individual risk in mean field control with application to automated demand response},
  author={Chen, Yue and others},
  booktitle={53rd IEEE Conf. on Decision and Control},
  pages={6425--6432},
  year={2014},
  organization={IEEE}
}

% @misc{openadr,
%   title = {OpenADR 2.0 Demand Response Program Implementation Guide},
%   howpublished = {\url{https://www.openadr.org/assets/openadr-drprogramguide-v1.0.pdf}}
% }


% @misc{condison,
%   title = {2011--2021 Demand Response event history book},
%   howpublished = {\url{https://www.coned.com/-/media/files/coned/documents/save-energy-money/rebates-incentives-tax-credits/smart-usage-rewards/demand-response-events.pdf?la=en.}}
% }

@article{meyn2015ancillary,
  title={Ancillary service to the grid using intelligent deferrable loads},
  author={Meyn, Sean P and others},
  journal={IEEE Trans. on Automatic Control},
  volume={60},
  number={11},
  pages={2847--2862},
  year={2015},
  publisher={IEEE}
}


@inproceedings{hao2012demand,
  title={How demand response from commercial buildings will provide the regulation needs of the grid},
  author={Hao, He and others},
  booktitle={2012 50th annual Allerton Conf. on communication, control, and computing (Allerton)},
  pages={1908--1913},
  year={2012},
  organization={IEEE}
}



@inproceedings{koch2011modeling,
  title={Modeling and control of aggregated heterogeneous thermostatically controlled loads for ancillary services},
  author={Koch, Stephan and others},
  booktitle={Proc. PSCC},
  pages={1--7},
  year={2011},
  organization={Citeseer}
}



@article{todorov2006linearly,
  title={Linearly-solvable Markov decision problems},
  author={Todorov, Emanuel},
  journal={Advances in neural information processing systems},
  volume={19},
  year={2006}
}

@incollection{chertkov2018ensemble,
  title={Ensemble control of cycling energy loads: Markov decision approach},
  author={Chertkov, Michael and others},
  booktitle={Energy Markets and Responsive Grids},
  pages={363--382},
  year={2018},
  publisher={Springer}
}


@article{hassan2020stochastic,
  title={Stochastic and distributionally robust load ensemble control},
  author={Hassan, Ali and others},
  journal={IEEE Trans. on Power Systems},
  volume={35},
  number={6},
  year={2020},
  publisher={IEEE}
}


@inproceedings{pop2019markov,
  title={A Markov process approach to ensemble control of smart buildings},
  author={Pop, Roman and others},
  booktitle={IEEE Milan PowerTech},
  pages={1--6},
  year={2019},
  organization={IEEE}
}






@article{wan2021distributed,
  title={Distributed algorithms for linearly-solvable optimal control in networked multi-agent systems},
  author={Wan, Neng and others},
  journal={arXiv preprint arXiv:2102.09104},
  year={2021}
}




@article{lobel2010distributed,
  title={Distributed subgradient methods for convex optimization over random networks},
  author={Lobel, Ilan and Ozdaglar, Asuman},
  journal={IEEE Trans. on Automatic Control},
  volume={56},
  number={6},
  pages={1291--1306},
  year={2010},
  publisher={IEEE}
}


@article{jakovetic2014fast,
  title={Fast distributed gradient methods},
  author={Jakoveti{\'c}, Du{\v{s}}an and others},
  journal={IEEE Trans. on Automatic Control},
  volume={59},
  number={5},
  pages={1131--1146},
  year={2014},
  publisher={IEEE}
}


@article{zhang2014online,
  title={Online optimal generation control based on constrained distributed gradient algorithm},
  author={Zhang, Wei and others},
  journal={IEEE Trans. on Power Systems},
  volume={30},
  number={1},
  pages={35--45},
  year={2014},
  publisher={IEEE}
}



@article{kullback1951information,
  title={On information and sufficiency},
  author={Kullback, Solomon and Leibler, Richard A},
  journal={The annals of mathematical statistics},
  volume={22},
  number={1},
  pages={79--86},
  year={1951},
  publisher={JSTOR}
}  
  
% \bibitem{KLD}
% S. Kullback, R. Leibler, ``On Information and Sufficiency," in \textit{The Annals of Mathematical Statistics}, 1951, 22(1), pp.79–86.
 
%  \bibitem{convexopt}
% S. Boyd, and L. Vandenberghe, ``Convex optimization," \textit{Cambridge university press}, 2004.

@book{greenberg2012introduction,
  title={Introduction to Bayesian econometrics},
  author={Greenberg, Edward},
  year={2012},
  publisher={Cambridge University Press}
}


@book{prohorov1969probability,
  title={Probability theory: basic concepts, limit theorems, random processes},
  author={Prohorov, Yurii Vasil'evich and others},
  volume={18},
  year={1969},
  publisher={Springer}
}





@article{hassan2020hierarchical,
  title={A hierarchical approach to multienergy demand response: From electricity to multienergy applications},
  author={Hassan, Ali and others},
  journal={Proc. of the IEEE},
  volume={108},
  number={9},
  pages={1457--1474},
  year={2020},
  publisher={IEEE}
}






% \bibitem{data1}
% A. Hassan, S. Acharya, M. Chertkov, D. Deka, and Y. Dvorkin, ``A hierarchical approach to multienergy demand response: From electricity to multienergy applications,” in \textit{Proc. of the IEEE}, 2020, 108(9), pp.1457-1474.



% \bibitem{data2}
% Consolidated Edison. [Online]. Available: https://www.coned.com/-/media/files/coned/documents/save-energy-money/rebates-incentives-tax-credits/smart-usage-rewards/demand-response-events.pdf?la=en


